Towards Robust Recommender Systems via Triple Cooperative Defense

Recommender systems are often susceptible to well-crafted fake profiles, leading to biased recommendations. The wide application of recommender systems makes studying the defense against attack necessary. Among existing defense methods, data-processing-based methods inevitably exclude normal samples, while model-based methods struggle to enjoy both generalization and robustness. Considering the above limitations, we suggest integrating data processing and robust model and propose a general framework, Triple Cooperative Defense (TCD), which cooperates to improve model robustness through the co-training of three models. Specifically, in each round of training, we sequentially use the high-confidence prediction ratings (consistent ratings) of any two models as auxiliary training data for the remaining model, and the three models cooperatively improve recommendation robustness. Notably, TCD adds pseudo label data instead of deleting abnormal data, which avoids the cleaning of normal data, and the cooperative training of the three models is also beneficial to model generalization. Through extensive experiments with five poisoning attacks on three real-world datasets, the results show that the robustness improvement of TCD significantly outperforms baselines. It is worth mentioning that TCD is also beneficial for model generalizations.

==> Dockerfile <==
FROM reitzig/texlive-base:2021.5
RUN apk update && apk add --no-cache bash perl python3 py3-pip
RUN pip3 install pygments

# Emulate "Install dependencies" of "entrypoint work ..."
RUN tlmgr update --self --repository https://mirror.mwt.me/ctan/systems/texlive/tlnet
COPY Texlivefile /work/src
RUN xargs tlmgr install --repository https://mirror.mwt.me/ctan/systems/texlive/tlnet < "/work/src/Texlivefile" && \
    sha256sum "/work/src/Texlivefile" > "/work/tmp/Texlivefile.sha" && \
#
# make latexmk and texlogsieve available
    cp /usr/local/texlive/2021/bin/x86_64-linuxmusl/latexmk /usr/local/bin && \
    cp /usr/local/texlive/2021/bin/x86_64-linuxmusl/texlogsieve /usr/local/bin && \
# use latest texlogsieve
    cd /usr/local/bin && wget https://gitlab.com/lago/texlogsieve/-/raw/main/texlogsieve?inline=false


==> latexmkrc <==
# `-file-line-error` is similar to `--interaction nonstopmode`, but shows the concrete line number
# Remove it, it you want lualatex to stop on errors
$pdflatex = 'pdflatex --shell-escape --interaction nonstopmode --synctex=-1 %O %S | texlogsieve';

#Use SumatraPDF instead of the default PDF viewer
$pdf_previewer = 'start "C:\Program Files\SumatraPDF\SumatraPDF.exe"';

#SumatraPDF updates automatically
$preview_mode = 0;

#automatically call lualatex/pdflatex (instead of latex)
$pdf_mode = 1;

add_cus_dep('glo', 'gls', 0, 'run_makeglossaries');
add_cus_dep('acn', 'acr', 0, 'run_makeglossaries');

sub run_makeglossaries {
  if ( $silent ) {
    system "makeglossaries", "-q", $_[0];
  }
  else {
    system "makeglossaries", $_[0];
  };
}

# enable deletion of *.bbl when calling "latexmk -c"
$bibtex_use = 2;

#remove more files than in the default configuration
@generated_exts = qw(acn acr alg aux code ist fls glg glo gls glsdefs idx ind lof lot out thm toc tpt wrt upa upb synctex);
$clean_ext .= ' %R.ist %R.xdy';

